On monitoring development indicators using high resolution satellite images

We develop a machine learning based tool for accurate prediction of socio-economic indicators from daytime satellite imagery. The diverse set of indicators are often not intuitively related to observable features in satellite images, and are not even always well correlated with each other. Our predictive tool is more accurate than using night light as a proxy, and can be used to predict missing data, smooth out noise in surveys, monitor development progress of a region, and flag potential anomalies. Finally, we use predicted variables to do robustness analysis of a regression study of high rate of stunting in India.

==> assetmodel.tex <==
\section{Asset model creation}

We derive our asset indicators from the {\it Houselisting and Housing} data (Table HH-14) of Census 2011 \citep{census} as indicated in Table \ref{table:assets}.

\begin{table}[ht]
\centering
\caption{Asset indicators aggregated from village level Census 2011 data}
\label{table:assets}
{\tiny
\begin{tabular}{|l|l|l|}
\hline
Indicator & Description (\% of houses in the village with) & Aggregated from columns \\
\hline \hline 
electronics & radio/transistor/tv/laptop & ([128]+[129]+[130]+[131)]/3\\ \hline
water-treated & water from treated source/covered well/ tube-well & [72]+[74]+[77] \\  \hline
water-untreated & water from untreated source/uncovered well & [73]+[75]\\  \hline
water-natural & drinking water from ponds/rivers/lakes & [76]+[78]+[79]+[80]+[81] \\  \hline
light from electricity &  from grid/solar & [85]+[87] \\  \hline
light from oil & kerosene/other oil & [86]+[88]+[89] \\  \hline
has-phone &  land-line/mobile/both & [132]+[133]+[134] \\  \hline
transport-cycle &  cycle & [135] \\  \hline
transport-motorized &  motorcycle/scooter/car/jeep & [136]+[137] \\  \hline
no-assets & no assets (cycle/phone etc.) & [139] \\  \hline
banking-services & availing banking services & [127] \\  \hline
cook-fuel-processed &  LPG/electric stove etc. & [113]+[114]+[115]\\   \hline
bathroom-within & bathroom within premises & [103]+[104] \\  \hline
rooms-under-3 &  less than 3 rooms & [49]+[50]+[51] \\  \hline
household-size-under-5 & less than 5 family members & [56]+[57]+[58]+[59] \\  \hline
permanent-house & permanent house & [140] \\  \hline
\end{tabular}
}
\end{table}

\citep{Jean790} used the first principal component of the data as the target of the regression.  However, we find that our manual aggregation gives better regression accuracy than using the linear principal component analysis (PCA) for dimensionality reduction.  Though the leading principal components capture high variance in the data, other components may be equally important for economic analysis.

